FLUTE: Figurative Language Understanding through Textual Explanations

Figurative language understanding has been recently framed as a recognizing textual entailment (RTE) task (a.k.a. natural language inference, or NLI). However, similar to classical RTE/NLI datasets, the current benchmarks suffer from spurious correlations and annotation artifacts. To tackle this problem, work on NLI has built explanation-based datasets such as e-SNLI, allowing us to probe whether language models are right for the right reasons.Yet no such data exists for figurative language, making it harder to assess genuine understanding of such expressions. To address this issue, we release FLUTE, a dataset of 9,000 figurative NLI instances with explanations, spanning four categories: Sarcasm, Simile, Metaphor, and Idioms. We collect the data through a model-in-the-loop framework based on GPT-3, crowd workers, and expert annotators. We show how utilizing GPT-3 in conjunction with human annotators (novices and experts) can aid in scaling up the creation of datasets even for such complex linguistic phenomena as figurative language. The baseline performance of the T5 model fine-tuned on FLUTE shows that our dataset can bring us a step closer to developing models that understand figurative language through textual explanations.

==> comments.tex <==
%We present \flute, a benchmark dataset containing <literal, figurative> sentence pairs, similar to NLI datasets (i.e., benchmark containing both entailment and contradiction pairs)  along with their explanations. The benchmark dataset spans across four different types of figurative language: Sarcasm, Simile, Metaphor, and Idiom. Creating a dataset of such creativity and diversity at scale, especially when it comes to figurative language, can be difficult, however. Owing to the difficulty in controlling the quality of free-form annotations, we resort to the \textit{model-in-the-loop framework}.
% talk about \cite{wiegreffe2021reframing} in previous work


%Next, to measure how LMs can correctly classify figurative instances from literal instances as well as generate correct explanations we propose a task inspired by instruction-based learning \cite{mishra2021cross,sanh2021multitask,wei2021finetuned} and train a T5 \cite{raffel2019exploring} model to jointly predict the label and explanation. In particular, we train two variants: (i) T5 trained on e-SNLI dataset \cite{NEURIPS2018_4c7a167b} (ii) T5 trained on \flute and test on a test set collected from \flute. 


%\citet{NEURIPS2018_4c7a167b} released the largest data for Natural Language explanations for NLI tasks. Since we do not deal with the \textit{neutral} class we discard data for those instance and train text-to-text models on the rest of the data. Inspired by recent progress in instruction based learning \cite{mishra2021cross,sanh2021multitask,wei2021finetuned} we frame our task in form of natural language instruction and train a T5 \cite{raffel2019exploring} model that jointly predicts the label and explanation. 
%In particular we train T5 models in 2 settings i) T5 trained on eSNLI ii) T5 trained on our data FLUTE. Additionally we also use as a baseline the current state-of-art for Natural Language Explanations by \citet{majumder2021rationale} which infuse commonsense knowledge from external resources.
%SM-f I am not sure if needed in intro
%We apply (i) an ensemble of automatic evaluation metrics that has been found to correlate better with human judgement \cite{kayser2021vil} i.e., BERTScore \cite{zhang2019bertscore} and BLEURT \cite{sellam2020bleurt}. (ii) Simulatability — the difference between task accuracy when the NLE is given as input vs. when it is not.
%tc reads perfect :) its short and crisp

%(ii) We highlight the challenges in assembling such a dataset for creative NLP tasks. \textit{Model-in-the-loop} framework allows for scaling up the annotation process without compromising quality. Our approach relies on the ability of language models to generate creative, diverse, and high quality examples using a few-shot prompting approach for GPT-3 with minimal human involvement.

%(iii) We conduct experiments using SOTA text-to-text generation models using e-SNLI and \flute. Automatic metrics show  model trained on the e-SNLI benchmark generalizes poorly on NLI pairs containing Figurative language. On the contrary, model fine-tuned on \flute produce higher quality explanations in terms of both automatic metrics and human evaluation (MTurk based evaluation, see Section \ref{section:eval}).

% apply (i) an ensemble of automatic evaluation metrics that has been found to correlate better with human judgement \cite{kayser2021vil} i.e., BERTScore \cite{zhang2019bertscore} and BLEURT \cite{sellam2020bleurt}. (ii) Simulatability — the difference between task accuracy when the NLE is given as input vs. when it is not. 

%SM-f seems redundant with description in each subsections
%For simile, metaphor, and idiom we leverage few-shot learning capabilities of GPT-3 to generate paraphrases (entailment premises) and contradictions (contradiction premises). We base these data on existing figurative language datasets. For sarcasm, we start with literal sentences from the Empathetic Dialogue Dataset \cite{rashid-etal-2021-towards} and generate paraphrases (entailment hypotheses) using GPT-3. Then, we ask crowdworkers to make minimal edits in these paraphrases to create sarcastic sentences (contradiction hypothesis).

%For generations, we rely on few-shot learning capabilities of GPT-3 \cite{brown2020language}. We provide a natural language instruction along with several examples of the task in each prompt. Each data instance and output from GPT-3 has been verified by three experts who have a strong background in figurative language and linguistics.
%We describe the methods for creating the Literal-Figurative pairs in detail in this section. In the case of metaphors, similes, and idioms, we create <literal, figurative> sentence pairs based on previously released datasets (details can be found in the following sections). For instance, given an example of a simile, we create a literal and a contradiction counterpart using the model-in-the-loop framework. On the contrary, for sarcasm, we start with a literal sentence and then generate its sarcastic rephrase. This is mainly because, although prior research \cite{chakrabarty-etal-2021-figurative} has released <literal,sarcastic> sentence pairs for RTE task, they are based on Twitter dataset, which is noisy, not diverse, hence often not usable. It should be noted we created these datatsets using GPT-3 and each and every sample was verified by 3 experts. Our experts have strong academic background in Figurative Language and Linguistics and are L1 english speakers.We detail the data creation process(s) in the following sub-sections. 
%\Smara{Hm, were all experts native speakers?}
 
%\Smara{There are some repetitive things in Sarcasm. Also The Idioms/Metaphor/Simile need a Figure simukar to Sarcasm where you put all of them, emphasizing that here Fig Language is Given and GPT-3 used for paraphrase/Contratition. In Sarcasm is not the case. I would also like to see in Fig the Prompts fro GPT-3... It is an important part of data creation. As is now, I have a hard time understing what was done. } 

%Prior work \cite{chakrabarty-etal-2021-figurative,ghosh-etal-2020-interpreting} released datasets of <literal, sarcastic> sentence pairs for the RTE task.
% , where human annotators rephrased sarcastic sentences to represent their literal intended meaning. 
% However, the majority of the literal sentences in these datasets use lexical antonyms (``flattering'' $\rightarrow$ ``disgusting'') or negations (``is great'' $\rightarrow$ ``is not great'') to represent the intended meaning. 
%The performance of transformer-based language models for sarcastic classification is near-perfect (95\%) because spurious cues, e.g. the use of lexical antonyms or negation word like \emph{not}, provide unfair advantages \cite{chakrabarty-etal-2021-figurative}.  

%in association with a given emotion label. 
% To address these issues and to provide higher quality data, we take the opposite approach, i.e., given a literal sentence we generate its sarcastic paraphrase written by crowd workers. Jointly modeling emotion and sarcasm has shown to be beneficial for sarcasm detection \cite{chauhan-etal-2020-sentiment} and thus we select the literal sentences from the Empathetic Dialogue dataset \cite{rashkin-etal-2019-towards}. Here, each conversation in the dataset is grounded to a situation, in association with a given emotion label. 

%SM-f I capture this above. 
%We experimented with generating sarcastic utterances directly via few-shot prompting using GPT-3, but the generations were problematic. First, they lacked semantic consistency, i.e, the generated sarcasm would be very different from the literal input. Second, they contained social biases, stereotypes, or toxic content. We also experimented with crowd workers, however, even with rigorous checks and qualification rounds we failed to recruit enough workers who were creative and consistent to generate sarcastic utterances at scale. This led us to decompose our task into two subtasks (Figure \ref{humanai}). In the first subtask, we generate a paraphrase from the literal text, and in the second, we generate a sarcastic sentence from the paraphrase.

% We also experimented with crowd workers, however, even with rigorous checks and qualification rounds we failed to recruit enough workers who were creative and consistent to generate sarcastic utterances at scale. 

% We input <literal sentence, emotion> pairs from the Empathetic Dialogue dataset and use few-shot prompting with GPT-3 \cite{brown2020language} to generate paraphrases. 

% The input literal sentences are from the Empathetic Dialogue dataset and they are already labeled with emotion. We generate paraphrase of these literal inputs by including the emotion in the prompt and use the few-shot learning framework of GPT3 \cite{brown2020language}. In particular, we prompt the model with natural language instruction to generate a paraphrase followed by a few demonstrative examples of <Literal, Emotion, Paraphrase>. 
% Next, we generate new paraphrases for different literal inputs through nucleus sampling. 



% Finally, starting from the 1,339 seed literal sentence from the Empathetic Dialogue dataset we generate 1,339 new paraphrases.   
%Observe that adding the emotion to the prompt for GPT-3 has helped the Turkers to apply a lexical antonym by converting ``annoying'' $\rightarrow$ ``pleasant'', thus generating a sarcastic instance.
%For instance, an example in Table \ref{sarc_subtasks} shows how simply by introducing a lexical antonym - \textbf{pleasant} - we can generate a sarcastic sentence.% 1,500 NLI instances  



% The simile portion of our data consists of sentences containing simile that are collected from previously released figurative language datasets \cite{10.1162/tacl_a_00478,chakrabarty-etal-2021-figurative,https://doi.org/10.48550/arxiv.2204.12632}.
% % \Smara{Maybe say 750 at the end, as the process first does 720 then filter to 642 then add 108 and is confusing. So sat the resulting number at the end of section}

% %(See Table \ref{table:simile_para_ex}, Row (H) and Row (P))

% \paragraph{Paraphrases} A simile typically has a subject and an object compared using a property. We first extract the <simile, property> pairs from the related datasets and convert them to their literal paraphrases using GPT-3, which replaces the \emph{object of comparison} with the property of comparison. To ensure semantic consistency during paraphrase generation we also provide the simile \emph{property} in the prompt. For instance, for the simile in Table \ref{table:data}, ``In fact the assembly hall was now like a steam sauna'' the object \emph{steam sauna} is replaced with its property \emph{hot and moist} to convert the simile into its paraphrase ``The assembly hall was now hot and moist, more so than usual'' (See Fig \ref{fig:architecture_allfig}).
% % Table \ref{table:data} shows the paraphrased literal version.
% We use this $<$simile, literal paraphrase$>$ pairs as entailment instances.  Three experts verify each paraphrase generated by GPT-3, resulting in 720 $<$<simile, literal entailment$>$ tuples that were deemed satisfactory by all the three experts.


% \paragraph{Contradictions} Once $<$simile, literal entailment$>$ pairs are verified, we again use GPT-3 to generate contradictions from the paraphrased sentence with respect to the simile's property. The experts verified 720 contradictions generated by GPT-3, out of which 642 <literal paraphrase, literal contradiction> tuples were deemed satisfactory. We further selected 108 challenging <simile, literal entailment, literal contradiction> instances from \newcite{https://doi.org/10.48550/arxiv.2204.12632}, defined by low RoBERTa logit of the correct option (see section \ref{subsubsection:simchallenge} for details), to complete our data to 750 pairs, i.e. 1,500 NLI instances. 
% % For an overview illustration of the pipeline, see Figure \ref{fig:simile_chart} in the Appendix. 
% All prompts are available on GitHub as well as in Appendix \ref{sec:appendix}.

% The simile example in Figure \ref{table:data} demonstrates an example from our data. 
% \debanjanin{explanation needed that describe the simile property thing.}

%The statistics for the metaphor partition of our dataset is shown in Table \ref{table:simile_para_ex}. We follow the following steps to create the metaphor dataset. 

% The metaphor portion of our data consists of sentences containing metaphors that are collected from previously released datasets \cite{chakrabarty-etal-2021-figurative,bigbench,stowe-etal-2022-impli}. We follow the same procedure as Simile as pointed in Figure \ref{fig:architecture_allfig}.

% third section of \flute comprises of 750 examples of metaphors with their corresponding (a)  literal entailment (b) contradictory counterparts, respectively. We follow the following steps to create the metaphor dataset.  

\iffalse

\begin{table}[htbp]
\centering
\small
\renewcommand{\arraystretch}{1.2}
\begin{tabular}{|l|l|}
\hline
Metaphor                                                         & The tax cut will \textit{uplift} the economy                                                                                       \\ \hline
\begin{tabular}[c]{@{}l@{}}Original\\ Entailment\end{tabular}    & The tax cut will help the economy                                                                                         \\ \hline
\begin{tabular}[c]{@{}l@{}}GPT-3\\ Entailment\end{tabular}        & \begin{tabular}[c]{@{}l@{}}With money saved from tax cuts, \\ the economy will surely be improved.\end{tabular} \\ \hline\hline
Metaphor                                                         & \begin{tabular}[c]{@{}l@{}}He \textit{absorbed} the knowledge or beliefs \\ of his tribe\end{tabular}                               \\ \hline
\begin{tabular}[c]{@{}l@{}}Original\\ Non entailment\end{tabular} & He absorbed the beverages of his tribe                                                                                    \\ \hline
\begin{tabular}[c]{@{}l@{}}GPT-3\\ Contradiction\end{tabular}     & \begin{tabular}[c]{@{}l@{}}He utterly decimated his tribe’s most\\ deeply held beliefs.\end{tabular}                      \\ \hline
\end{tabular}
\caption{Example of Metaphors and entailment and contradiction (from prior work and generated for this paper.)}
\label{table:metaphor_ent_ex}
\end{table}


\fi

%which means there is no direct contradiction with respect to the metaphor (rather, this pair would be classified as non-entailment). 
%SM-f Why are we talking about contratictions in the entailement case, I commented out and replaced. 

% Next, we prompt the GPT-3 model to generate paraphrases of the metaphors given a few demonstrative examples of the pairs of $<$metaphor, literal entailment$>$ from the data sources. Although, the original datasets contain $<$metaphor, literal entailment$>$ pairs we chose to use GPT-3 for the following reasons: (a) not all metaphor examples \cite{bigbench} contain $<$metaphor,literal entailment$>$ pairs as inputs (b) often, the literal entailment is just a  minimal modification (one-word edit) of the metaphor sentence.

%Consider the examples in Table \ref{table:metaphor_ent_ex}. In case of entailment, notice  the original entailed sentence ``The tax cut \dots'' edits only one word from the metaphor whereas the GPT-3 generated example is more meaningful to the context.

% The pair of metaphors with the original entailment/non entailment are from the datasets we use. 

% but this time we prompt the model with a few examples of metaphors and their original contradiction pairs
